QUBIC VI: cryogenic half wave plate rotator, design and performances

Inflation Gravity Waves B-Modes polarization detection is the ultimate goal of modern large angular scale cosmic microwave background (CMB) experiments around the world. A big effort is undergoing with the deployment of many ground-based, balloon-borne and satellite experiments using different methods to separate this faint polarized component from the incoming radiation. One of the largely used technique is the Stokes Polarimetry that uses a rotating half-wave plate (HWP) and a linear polarizer to separate and modulate the polarization components with low residual cross-polarization. This paper describes the QUBIC Stokes Polarimeter highlighting its design features and its performances. A common systematic with these devices is the generation of large spurious signals synchronous with the rotation and proportional to the emissivity of the optical elements. A key feature of the QUBIC Stokes Polarimeter is to operate at cryogenic temperature in order to minimize this unwanted component. Moving efficiently this large optical element at low temperature constitutes a big engineering challenge in order to reduce friction power dissipation. Big attention has been given during the designing phase to minimize the differential thermal contractions between parts. The rotation is driven by a stepper motor placed outside the cryostat to avoid thermal load dissipation at cryogenic temperature. The tests and the results presented in this work show that the QUBIC polarimeter can easily achieve a precision below 0.1{\deg} in positioning simply using the stepper motor precision and the optical absolute encoder. The rotation induces only few mK of extra power load on the second cryogenic stage (~ 8 K).

==> authors_08.tex <==
% authors.tex :  this file automatically generated by author_list.py
%% DO NOT EDIT.  It will be clobbered next time you run author_list.py
\author[1,2]{G.~D'Alessandro}
\author[1,2]{F.~Columbro}
\author[1,2]{L.~Mele}
\author[1]{G.~Amico}
\author[1,2]{E.S.~Battistelli}
\author[1,2]{A.~Coppolecchia}
\author[1,2]{P.~de~Bernardis}
\author[1,2]{M.~De~Petris}
\author[3]{M.~Gonz\a'{a}lez}
\author[4]{L.~Grandsire}
\author[4]{J.-Ch.~Hamilton}
\author[1,2]{L.~Lamagna}
\author[1,2]{S.~Masi}
\author[5]{S.~Marnieros}
\author[6,7]{A.~Mennella}
\author[1,2]{A.~Paiella}
\author[1,2]{F.~Piacentini}
\author[4]{M.~Piat}
\author[12]{G.~Pisano}
\author[4]{G.~Stankowiak}
\author[8]{C.~O'Sullivan}
\author[9]{A.~Tartari}
\author[4]{J.-P.~Thermeau}
\author[4,10]{S.A.~Torchinsky}
\author[4]{F.~Voisin}
\author[11,7]{M.~Zannoni}
\author[12]{P.~Ade}
\author[13]{J.G.~Alberro}
\author[14]{A.~Almela}
\author[3]{L.H.~Arnaldi}
\author[5]{D.~Auguste}
\author[15]{J.~Aumont}
\author[16]{S.~Azzoni}
\author[11,7]{S.~Banfi}
\author[17]{B.~B\a'{e}lier}
\author[11,7]{A.~Ba\a`{u}}
\author[8]{D.~Bennett}
\author[5]{L.~Berg\a'{e}}
\author[15]{J.-Ph.~Bernard}
\author[6,7]{M.~Bersanelli}
\author[4]{M.-A.~Bigot-Sazy}
\author[18]{J.~Bonaparte}
\author[5]{J.~Bonis}
\author[19]{E.~Bunn}
\author[8]{D.~Burke}
\author[1]{D.~Buzi}
\author[6,7]{F.~Cavaliere}
\author[4]{P.~Chanial}
\author[4]{C.~Chapron}
\author[4]{R.~Charlassier}
\author[14]{A.C.~Cobos~Cerutti}
\author[20, 34]{G.~De~Gasperis}
\author[1,21]{M.~De~Leo}
\author[4]{S.~Dheilly}
\author[14]{C.~Duca}
\author[5]{L.~Dumoulin}
\author[14]{A.~Etchegoyen}
\author[18]{A.~Fasciszewski}
\author[14]{L.P.~Ferreyro}
\author[14]{D.~Fracchia}
\author[6,7]{C.~Franceschet}
\author[22]{M.M.~Gamboa Lerena}
\author[4]{K.M.~Ganga}
\author[14]{B.~Garc\a'{i}a}
\author[14]{M.E.~Garc\a'{i}a Redondo}
\author[5]{M.~Gaspard}
\author[8]{D.~Gayer}
\author[11,7]{M.~Gervasi}
\author[15]{M.~Giard}
\author[1]{V.~Gilles}
\author[4]{Y.~Giraud-Heraud}
\author[3]{M.~G\a'{o}mez Berisso}
\author[8]{M.~Gradziel}
\author[14]{M.R.~Hampel}
\author[5]{S.~Henrot-Versill\a'{e}}
\author[6,7]{F.~Incardona}
\author[5]{E.~Jules}
\author[4]{J.~Kaplan}
\author[23]{C.~Kristukat}
\author[4,24]{S.~Loucatos}
\author[5]{T.~Louis}
\author[25]{B.~Maffei}
\author[15]{W.~Marty}
\author[2]{A.~Mattei}
\author[26]{A.~May}
\author[26]{M.~McCulloch}
\author[14]{D.~Melo}
\author[15]{L.~Montier}
\author[4]{L.~Mousset}
\author[13]{L.M.~Mundo}
\author[8]{J.A.~Murphy}
\author[8]{J.D.~Murphy}
\author[11,7]{F.~Nati}
\author[5]{E.~Olivieri}
\author[5]{C.~Oriol}
\author[15]{F.~Pajot}
\author[11,7]{A.~Passerini}
\author[3]{H.~Pastoriza}
\author[2]{A.~Pelosi}
\author[4]{C.~Perbost}
\author[2]{M.~Perciballi}
\author[6,7]{F.~Pezzotta}
\author[26]{L.~Piccirillo}
\author[14]{M.~Platino}
\author[27]{G.~Polenta}
\author[4]{D.~Pr\a^{e}le}
\author[28]{R.~Puddu}
\author[15]{D.~Rambaud}
\author[29]{E.~Rasztocky}
\author[13]{P.~Ringegni}
\author[29]{G.E.~Romero}
\author[14]{J.M.~Salum}
\author[30]{A.~Schillaci}
\author[22, 35]{C.~Sc\a'{o}ccola}
\author[8,31]{S.~Scully}
\author[11]{S.~Spinelli}
\author[4]{M.~Stolpovskiy}
\author[14]{A.D.~Supanitsky}
\author[32]{P.~Timbie}
\author[6,7]{M.~Tomasi}
\author[33]{G.~Tucker}
\author[12]{C.~Tucker}
\author[6,7]{D.~Vigan\a`{o}}
\author[20]{N.~Vittorio}
\author[5]{F.~Wicek}
\author[26]{M.~Wright}
\author[2]{and A.~Zullo}



\affiliation[1]{Universit\a`{a} di Roma - La Sapienza}
\affiliation[2]{INFN Rome section}
\affiliation[3]{Centro At\a'{o}mico Bariloche and Instituto Balseiro (CNEA)}
\affiliation[4]{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France}
\affiliation[5]{Laboratoire de Physique des 2 Infinis Ir\a`{e}ne Joliot-Curie (CNRS-IN2P3, Universit\a'e Paris-Saclay)}
\affiliation[6]{Universita degli studi di Milano}
\affiliation[7]{INFN Milano-Bicocca}
\affiliation[8]{National University of Ireland, Maynooth}
\affiliation[9]{INFN - Pisa Section, 56127 Pisa, Italy}
\affiliation[10]{Observatoire de Paris, Université Paris Science et Lettres, F-75014 Paris, France}
\affiliation[11]{Universit\a`{a} di Milano - Bicocca}
\affiliation[12]{Cardiff University}
\affiliation[13]{GEMA (Universidad Nacional de La Plata)}
\affiliation[14]{Instituto de Tecnolog\a'{i}as en Detecci\a'{o}n y Astropart\a'{i}culas  (CNEA, CONICET, UNSAM)}
\affiliation[15]{Institut de Recherche en Astrophysique et Plan\a'{e}tologie, Toulouse (CNRS-INSU)}
\affiliation[16]{Department of Physics, University of Oxford}
\affiliation[17]{Centre de Nanosciences et de Nanotechnologies, Orsay}
\affiliation[18]{Centro At\a'{o}mico Constituyentes (CNEA)}
\affiliation[19]{University of Richmond, Richmond}
\affiliation[20]{Universit\a`{a} di Roma -  Tor Vergata}
\affiliation[21]{University of Surrey}
\affiliation[22]{Facultad de Ciencias Astron\a'{o}micas y Geof\a'{i}sicas (Universidad Nacional de La Plata)}
\affiliation[23]{Escuela de Ciencia y Tecnolog\a'{i}a (UNSAM) and Centro At\a'{o}mico Constituyentes (CNEA)}
\affiliation[24]{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affiliation[25]{Institut d'Astrophysique Spatiale, Orsay (CNRS-INSU)}
\affiliation[26]{University of Manchester}
\affiliation[27]{Italian Space Agency}
\affiliation[28]{Pontificia Universidad Catolica de Chile}
\affiliation[29]{Instituto Argentino de Radioastronom\a'{i}a (CONICET, CIC, UNLP)}
\affiliation[30]{California Institute of Technology}
\affiliation[31]{Institute of Technology, Carlow}
\affiliation[32]{University of Wisconsin, Madison}
\affiliation[33]{Brown University, Providence}
\affiliation[34]{INFN Sez. di Roma2}
\affiliation[35]{CONICET}







\emailAdd{giuseppe.dalessandro@uniroma1.it}
\emailAdd{ lorenzo.mele@roma1.infn.it}
\emailAdd{ fabio.columbro@roma1.infn.it}


==> authors_2.tex <==
% authors.tex :  this file automatically generated by author_list.py
%% DO NOT EDIT.  It will be clobbered next time you run author_list.py
\author[1]{G.~D'Alessandro}
\author[1]{L.~Mele}
\author[1]{F.~Columbro}
\author[1]{E.S.~Battistelli}
\author[2]{G.~Amico}
\author[1]{A.~Coppolecchia}
\author[3]{J.-Ch.~Hamilton}
\author[1]{P.~de~Bernardis}
\author[1]{M.~De Petris}
\author[1]{L.~Lamagna}
\author[1]{S.~Masi}
\author[1]{A.~Paiella}
\author[1]{F.~Piacentini}
\author[3]{M.~Piat}
\author[4]{S.A.~Torchinsky}
\author[5]{P.~Ade}
\author[6]{J.G.~Alberro}
\author[7]{A.~Almela}
\author[8]{L.H.~Arnaldi}
\author[9]{D.~Auguste}
\author[10]{J.~Aumont}
\author[11]{S.~Azzoni}
\author[12]{S.~Banfi}
\author[12]{A.~Ba\a`{u}}
\author[13]{B.~B\a'{e}lier}
\author[14]{D.~Burke}
\author[14]{D.~Bennett}
\author[9]{L.~Berg\a'{e}}
\author[10]{J.-Ph.~Bernard}
\author[15]{M.~Bersanelli}
\author[3]{M.-A.~Bigot-Sazy}
\author[16]{J.~Bonaparte}
\author[9]{J.~Bonis}
\author[6]{A.~Bottani}
\author[17]{E.~Bunn}
\author[2]{D.~Buzi}
\author[15]{F.~Cavaliere}
\author[3]{P.~Chanial}
\author[3]{C.~Chapron}
\author[3]{R.~Charlassier}
\author[7]{A.C.~Cobos~Cerutti}
\author[18]{G.~De Gasperis}
\author[2,31]{M.~De Leo}
\author[3]{S.~Dheilly}
\author[7]{C.~Duca}
\author[9]{L.~Dumoulin}
\author[19]{M.M.~Gamboa Lerena}
\author[8]{M.~Gonz\a'{a}lez}
\author[7]{A.~Etchegoyen}
\author[16]{A.~Fasciszewski}
\author[7]{L.P.~Ferreyro}
\author[7]{D.~Fracchia}
\author[15]{C.~Franceschet}
\author[3]{K.M.~Ganga}
\author[7]{B.~Garc\a'{i}a}
\author[7]{M.E.~Garc\a'{i}a Redondo}
\author[9]{M.~Gaspard}
\author[14]{D.~Gayer}
\author[12]{M.~Gervasi}
\author[10]{M.~Giard}
\author[2]{V.~Gilles}
\author[3]{Y.~Giraud-Heraud}
\author[8]{M.~G\a'{o}mez Berisso}
\author[14]{M.~Gradziel}
\author[3]{L.~Grandsire}
\author[8]{D.~Harari}
\author[9]{S.~Henrot-Versill\a'{e}}
\author[15]{F.~Incardona}
\author[9]{E.~Jules}
\author[3]{J.~Kaplan}
\author[20]{C.~Kristukat}
\author[3]{S.~Loucatos}
\author[9]{T.~Louis}
\author[21]{B.~Maffei}
\author[9]{S.~Marnieros}
\author[10]{W.~Marty}
\author[22]{A.~Mattei}
\author[11]{A.~May}
\author[11]{M.~McCulloch}
\author[11]{S.~Melhuish}
\author[15]{A.~Mennella}
\author[10]{L.~Montier}
\author[3]{L.~Mousset}
\author[6]{L.~M.~Mundo}
\author[14]{J.~A.~Murphy}
\author[14]{J.D.~Murphy}
\author[12]{F.~Nati}
\author[9]{E.~Olivieri}
\author[9]{C.~Oriol}
\author[14]{C.~O'Sullivan}
\author[10]{F.~Pajot}
\author[12]{A.~Passerini}
\author[8]{H.~Pastoriza}
\author[22]{A.~Pelosi}
\author[3]{C.~Perbost}
\author[22]{M.~Perciballi}
\author[15]{F.~Pezzotta}
\author[11]{L.~Piccirillo}
\author[5]{G.~Pisano}
\author[7]{M.~Platino}
\author[23]{G.~Polenta}
\author[3]{D.~Pr\a^{e}le}
\author[24]{R.~Puddu}
\author[10]{D.~Rambaud}
\author[6]{P.~Ringegni}
\author[25]{G.~E.~Romero}
\author[19]{C.~Sc\a'{o}ccola}
\author[3]{G.~Stankowiak}
\author[7]{J.M.~Salum}
\author[26]{A.~Schillaci}
\author[14]{S.~Scully}
\author[27]{S.~Spinelli}
\author[3]{M.~Stolpovskiy}
\author[7]{A.D.~Supanitsky}
\author[28]{A.~Tartari}
\author[29]{P.~Timbie}
\author[3]{J.-P.~Thermeau}
\author[15]{M.~Tomasi}
\author[30]{G.~Tucker}
\author[5]{C.~Tucker}
\author[15]{D.~Vigan\a`{o}}
\author[18]{N.~Vittorio}
\author[3]{F.~Voisin}
\author[9]{F.~Wicek}
\author[12]{M.~Zannoni}
\author[22]{and A.~Zullo}

\affiliation[1]{Universit\a`{a} di Roma - La Sapienza and INFN Rome section}
\affiliation[2]{Universit\a`{a} di Roma - La Sapienza}
\affiliation[3]{Astroparticule et Cosmologie, Paris  (CNRS-IN2P3, Universit\a'e de Paris)}
\affiliation[4]{Astroparticule et Cosmologie, Paris (Observatoire de Paris, CNRS/IN2P3, Universit\a'e de Paris)}
\affiliation[5]{Cardiff University}
\affiliation[6]{GEMA (Universidad Nacional de La Plata)}
\affiliation[7]{Instituto de Tecnolog\a'{i}as en Detecci\a'{o}n y Astropart\a'{i}culas  (CNEA, CONICET, UNSAM)}
\affiliation[8]{Centro At\a'{o}mico Bariloche and Instituto Balseiro (CNEA)}
\affiliation[9]{Laboratoire de Physique des 2 Infinis Ir\a`{e}ne Joliot-Curie (CNRS-IN2P3, Universit\a'e Paris-Saclay)}
\affiliation[10]{Institut de Recherche en Astrophysique et Plan\a'{e}tologie, Toulouse (CNRS-INSU)}
\affiliation[11]{University of Manchester}
\affiliation[12]{Universit\a`{a} di Milano - Bicocca and INFN Milano-Bicocca}
\affiliation[13]{Centre de Nanosciences et de Nanotechnologies, Orsay}
\affiliation[14]{National University of Ireland, Maynooth}
\affiliation[15]{Universita degli studi di Milano and INFN Milano}
\affiliation[16]{Centro At\a'{o}mico Constituyentes (CNEA)}
\affiliation[17]{University of Richmond, Richmond}
\affiliation[18]{Universit\a`{a} di Roma -  Tor Vergata}
\affiliation[19]{Facultad de Cs Astron\a'{o}micas y Geof\a'{i}sicas (Universidad Nacional de La Plata)}
\affiliation[20]{Escuela de Ciencia y Tecnolog\a'{i}a (UNSAM) and Centro At\a'{o}mico Constituyentes (CNEA)}
\affiliation[21]{Institut d'Astrophysique Spatiale, Orsay (CNRS-INSU)}
\affiliation[22]{INFN Rome section}
\affiliation[23]{Italian Space Agency}
\affiliation[24]{Pontificia Universidad Catolica de Chile}
\affiliation[25]{Instituto Argentino de Radioastronom\a'{i}a (CONICET, CIC)}
\affiliation[26]{California Institute of Technology}
\affiliation[27]{Universit\a`{a} di Milano - Bicocca}
\affiliation[28]{INFN - Pisa Section, 56127 Pisa, Italy}
\affiliation[29]{University of Wisconsin, Madison}
\affiliation[30]{Brown University, Providence}
\affiliation[31]{University of Surrey}























\emailAdd{giuseppe.dalessandro@uniroma1.it, lorenzo.mele@roma1.infn.it, fabio.columbro@roma1.infn.it}

==> authors_6_EdB.tex <==
% authors.tex :  this file automatically generated by author_list.py
%% DO NOT EDIT.  It will be clobbered next time you run author_list.py
\author[1,2]{G.~D'Alessandro}
\author[1,2]{L.~Mele}
\author[1,2]{F.~Columbro}
\author[1]{G.~Amico}
\author[1,2]{E.S.~Battistelli}
\author[1,2]{P.~de~Bernardis}
\author[1,2]{A.~Coppolecchia}
\author[1,2]{M.~De~Petris}
\author[3]{L.~Grandsire}
\author[3]{J.-Ch.~Hamilton}
\author[1,2]{L.~Lamagna}
\author[4]{S.~Marnieros}
\author[1,2]{S.~Masi}
\author[5,6]{A.~Mennella}
\author[7]{C.~O'Sullivan}
\author[1,2]{A.~Paiella}
\author[1,2]{F.~Piacentini}
\author[3]{M.~Piat}
\author[8]{G.~Pisano}
\author[1,2]{G.~Presta}
\author[9]{A.~Tartari}
\author[3,10]{S.A.~Torchinsky}
\author[3]{F.~Voisin}
\author[11,12]{M.~Zannoni}
\author[8]{P.~Ade}
\author[13]{J.G.~Alberro}
\author[14]{A.~Almela}
\author[15]{L.H.~Arnaldi}
\author[4]{D.~Auguste}
\author[16]{J.~Aumont}
\author[17]{S.~Azzoni}
\author[11,12]{S.~Banfi}
\author[11,12]{A.~Ba\a`{u}}
\author[18]{B.~B\a'{e}lier}
\author[7]{D.~Bennett}
\author[4]{L.~Berg\a'{e}}
\author[16]{J.-Ph.~Bernard}
\author[5,6]{M.~Bersanelli}
\author[3]{M.-A.~Bigot-Sazy}
\author[19]{J.~Bonaparte}
\author[4]{J.~Bonis}
\author[20]{E.~Bunn}
\author[7]{D.~Burke}
\author[1]{D.~Buzi}
\author[5,6]{F.~Cavaliere}
\author[3]{P.~Chanial}
\author[3]{C.~Chapron}
\author[3]{R.~Charlassier}
\author[14]{A.C.~Cobos~Cerutti}
\author[21,22]{G.~De~Gasperis}
\author[1,23]{M.~De~Leo}
\author[3]{S.~Dheilly}
\author[14]{C.~Duca}
\author[4]{L.~Dumoulin}
\author[14]{A.~Etchegoyen}
\author[19]{A.~Fasciszewski}
\author[14]{L.P.~Ferreyro}
\author[14]{D.~Fracchia}
\author[5,6]{C.~Franceschet}
\author[24,25]{M.M.~Gamboa Lerena}
\author[3]{K.M.~Ganga}
\author[14]{B.~Garc\a'{i}a}
\author[14]{M.E.~Garc\a'{i}a Redondo}
\author[4]{M.~Gaspard}
\author[7]{D.~Gayer}
\author[11,12]{M.~Gervasi}
\author[16]{M.~Giard}
\author[1,26]{V.~Gilles}
\author[3]{Y.~Giraud-Heraud}
\author[15]{M.~G\a'{o}mez Berisso}
\author[15]{M.~Gonz\a'{a}lez}
\author[7]{M.~Gradziel}
\author[14]{M.R.~Hampel}
\author[15]{D.~Harari}
\author[4]{S.~Henrot-Versill\a'{e}}
\author[5,6]{F.~Incardona}
\author[4]{E.~Jules}
\author[3]{J.~Kaplan}
\author[27]{C.~Kristukat}
\author[3,28]{S.~Loucatos}
\author[4]{T.~Louis}
\author[29]{B.~Maffei}
\author[16]{W.~Marty}
\author[2]{A.~Mattei}
\author[26]{A.~May}
\author[26]{M.~McCulloch}
\author[14]{D.~Melo}
\author[16]{L.~Montier}
\author[3]{L.~Mousset}
\author[13]{L.M.~Mundo}
\author[7]{J.A.~Murphy}
\author[7]{J.D.~Murphy}
\author[11,12]{F.~Nati}
\author[4]{E.~Olivieri}
\author[4]{C.~Oriol}
\author[16]{F.~Pajot}
\author[11,12]{A.~Passerini}
\author[15]{H.~Pastoriza}
\author[2]{A.~Pelosi}
\author[3]{C.~Perbost}
\author[2]{M.~Perciballi}
\author[5,6]{F.~Pezzotta}
\author[26]{L.~Piccirillo}
\author[14]{M.~Platino}
\author[1,30]{G.~Polenta}
\author[3]{D.~Pr\a^{e}le}
\author[31]{R.~Puddu}
\author[16]{D.~Rambaud}
\author[32]{E.~Rasztocky}
\author[13]{P.~Ringegni}
\author[32]{G.E.~Romero}
\author[14]{J.M.~Salum}
\author[1,33]{A.~Schillaci}
\author[24,25]{C.G.~Sc\a'{o}ccola}
\author[7,34]{S.~Scully}
\author[11]{S.~Spinelli}
\author[3]{G.~Stankowiak}
\author[3]{M.~Stolpovskiy}
\author[14]{A.D.~Supanitsky}
\author[3]{J.-P.~Thermeau}
\author[35]{P.~Timbie}
\author[5,6]{M.~Tomasi}
\author[8]{C.~Tucker}
\author[36]{G.~Tucker}
\author[5,6]{D.~Vigan\a`{o}}
\author[21]{N.~Vittorio}
\author[4]{F.~Wicek}
\author[26]{M.~Wright}
\author[2]{and A.~Zullo}


\affiliation[23]{University of Surrey, UK}
\affiliation[1]{Universit\a`{a} di Roma - La Sapienza, Roma, Italy}
\affiliation[31]{Pontificia Universidad Catolica de Chile, Chile}
\affiliation[36]{Brown University, Providence, USA}
\affiliation[12]{INFN sezione di Milano - Bicocca, 20216 Milano, Italy}
\affiliation[26]{University of Manchester, UK}
\affiliation[14]{Instituto de Tecnolog\a'{i}as en Detecci\a'{o}n y Astropart\a'{i}culas  (CNEA, CONICET, UNSAM), Argentina}
\affiliation[25]{CONICET, Argentina}
\affiliation[5]{Universit\a`{a} degli studi di Milano, Milano, Italy}
\affiliation[11]{Universit\a`{a} di Milano - Bicocca, Milano, Italy}
\affiliation[8]{Cardiff University, UK}
\affiliation[3]{Universit\'e de Paris, CNRS, Astroparticule et Cosmologie, F-75006 Paris, France}
\affiliation[30]{Italian Space Agency, Roma, Italy}
\affiliation[2]{INFN sezione di Roma, 00185 Roma, Italy}
\affiliation[9]{INFN sezione di Pisa, 56127 Pisa, Italy}
\affiliation[22]{INFN sezione di Roma2, 00133 Roma, Italy}
\affiliation[20]{University of Richmond, Richmond, USA}
\affiliation[13]{GEMA (Universidad Nacional de La Plata), Argentina}
\affiliation[33]{California Institute of Technology, USA}
\affiliation[18]{Centre de Nanosciences et de Nanotechnologies, Orsay, France}
\affiliation[29]{Institut d'Astrophysique Spatiale, Orsay (CNRS-INSU), France}
\affiliation[19]{Centro At\a'{o}mico Constituyentes (CNEA), Argentina}
\affiliation[24]{Facultad de Ciencias Astron\a'{o}micas y Geof\a'{i}sicas (Universidad Nacional de La Plata), Argentina}
\affiliation[32]{Instituto Argentino de Radioastronom\a'{i}a (CONICET, CIC, UNLP), Argentina}
\affiliation[28]{IRFU, CEA, Universit\'e Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\affiliation[7]{National University of Ireland, Maynooth, Ireland}
\affiliation[17]{Department of Physics, University of Oxford, UK}
\affiliation[16]{Institut de Recherche en Astrophysique et Plan\a'{e}tologie, Toulouse (CNRS-INSU), France}
\affiliation[6]{INFN sezione di Milano, 20133 Milano, Italy}
\affiliation[35]{University of Wisconsin, Madison, USA}
\affiliation[27]{Escuela de Ciencia y Tecnolog\a'{i}a (UNSAM) and Centro At\a'{o}mico Constituyentes (CNEA), Argentina}
\affiliation[15]{Centro At\a'{o}mico Bariloche and Instituto Balseiro (CNEA), Argentina}
\affiliation[21]{Universit\a`{a} di Roma ``Tor Vergata'', Roma, Italy}
\affiliation[10]{Observatoire de Paris, Universit\'e Paris Science et Lettres, F-75014 Paris, France}
\affiliation[34]{Institute of Technology, Carlow, Ireland}
\affiliation[4]{Laboratoire de Physique des 2 Infinis Ir\a`{e}ne Joliot-Curie (CNRS-IN2P3, Universit\a'e Paris-Saclay), France}


